Rough kernel hedging

Building on the functional-analytic framework of operator-valued kernels and un-truncated signature kernels, we propose a scalable, provably convergent signature-based algorithm for a broad class of high-dimensional, path-dependent hedging problems. We make minimal assumptions about market dynamics by modelling them as general geometric rough paths, yielding a fully model-free approach. Furthermore, through a representer theorem, we provide theoretical guarantees on the existence and uniqueness of a global minimum for the resulting optimization problem and derive an analytic solution under highly general loss functions. Similar to the popular deep hedging approach, but in a more rigorous fashion, our method can also incorporate additional features via the underlying operator-valued kernel, such as trading signals, news analytics, and past hedging decisions, closely aligning with true machine-learning practice.

==> old_proofs.tex <==
\newpage

\section{Old Proofs}

\begin{lemma}
    If $K(X,Y) = K_{sig}^{\text{It\^o}}(X,Y) Id_V$ then 
    \[
    \frac{1}{d} \E\left[ \int_0^T | Tr(K(X|_{0,t}, X|_{0,t})) |  Tr(d[X,X]_t) \right] =  \E\left[ K_{sig}^{\text{It\^o}}(X,X)_{T,T} - 1 \right]
    \]
    Moreover, when $[X,X]_t$ is deterministic, one has
    \[
    \E\left[ K_{sig}^{\text{It\^o}}(X,X)_{T,T} - 1 \right] = \sum_{|I|>0} Sig([X])_{0,T}^I < \infty
    \]
    where $[X]_t = diag([X,X]_t)$. 
\end{lemma}
{Thus by Proposition \ref{prop:Phi_stoch} the stochastic It\^o feature map is well defined.}
\begin{proof}
    One has 
    \[
    | Tr(K(X|_{0,t}, X|_{0,t})) | = d \cdot K_{sig}^{\text{It\^o}}(X,X)_{t,t}
    \]
    hence
    \[
    \frac{1}{d} \int_0^T | Tr(K(X|_{0,t}, X|_{0,t})) |  Tr(d[X,X]_t)
        = \int_0^T K_{sig}^{\text{It\^o}}(X,X)_{t,t}  Tr(d[X,X]_t) 
    \]

    Now notice how 
    \begin{align*}
        \E\left[ \int_0^T (Sig^{\text{It\^o}}(X)^I_{0,t})^2 Tr(d[X,X]_t) \right]
        = &
        \E\left[ \norm{ \int_0^T Sig^{\text{It\^o}}(X)^I_{0,t} \D X_t  }^2 \right]
        \\
        = &
        \sum_{k=1}^d \E\left[ \left( Sig^{\text{It\^o}}(X)^{Ik}_{0,T} \right) ^2 \right]
    \end{align*}
    hence summing over $I \in \mathbb{W}_d$
    \begin{align*}
        \E\left[ \int_0^T K_{sig}^{\text{It\^o}}(X,X)_{t,t}  Tr(d[X,X]_t) \right]
        = & \E\left[ K_{sig}^{\text{It\^o}}(X,X)_{T,T} - 1 \right]
    \end{align*}

    At the same time note that if $[X,X]$ is deterministic then
    \begin{align*}
        \E\left[ K_{sig}^{\text{It\^o}}(X,X)_{T,T}\right] 
        = & 1 + \E\left[ \int_0^T K_{sig}^{\text{It\^o}}(X,X)_{t,t}  Tr(d[X,X]_t) \right]
        \\
        = & 1 + \int_0^T \E\left[ K_{sig}^{\text{It\^o}}(X,X)_{t,t} \right] Tr(d[X,X]_t) 
    \end{align*}
    meaning that $Y_s := \E\left[ K_{sig}^{\text{It\^o}}(X,X)_{s,s}\right]$ solves
    \[
    Y_t = 1 + \sum_{i=1}^d \int_0^t Y_s d[X^i]_s
    \]
    which has, as needed, explicit solution written as
    \[
    Y_t = \sum_{I} Sig([X])^I_{0,t}
    \]
\end{proof}


\begin{lemma}
    Let $p = 1$ and $X \in \Omega_T := C^\alpha([0,T];\bR^d)$. 
    If the path
    \begin{equation}
        [0,T] \ni s \mapsto K(X|_{[0,s]}, \cdot) \in \cL(\bR^d, \cH_{K}) 
    \end{equation}
    is continuous, then for any $f \in \cH_{K}$ 
    \begin{equation}\label{eqn:core_swap_1}
        \int_0^T \left\langle f(X|_{[0,t]}), \D X_t \right\rangle_{\bR^d} = \left\langle f, \Phi_X \right\rangle_{\cH_{K}}
    \end{equation}
    where the element $\Phi_X \in \cH_{K}$ is defined as the Bochner Integral
    \begin{equation}
        \Phi_X := \int_0^T K(X|_{[0,t]}, \cdot) \D X_t.
    \end{equation}
\end{lemma}

% \Cris{We should look at this proof together. Notation is not clear.}

\begin{proof}
    
    Fix $X \in \Omega_T$. Fix a partition $\cD := \{0=t_0 \leq \dots \leq t_D = T\}$ and define 
    \[
    J_{\cD} := \sum_{i=0}^{D-1} K(X|_{[0,t_i]},\cdot)[X_{t_{i+1}} - X_{t_{i}}] \in \cH_{K}
    \]

    Let $\cD' := \{ 0=s_0 \leq \dots \leq s_{D'} = T \}$ be a refinement of $\cD$ \emph{i.e.} there exists a strictly increasing function $\xi : [D] \to [D']$ such that $\xi(0) = 0$ and $s_{\xi(i)} = t_i$.
    Let $\tilde{\xi} : [D'] \to [\cD]$ be the map $\tilde{\xi}(j) = \xi(\max \{ i \in [D] : \xi(i) \leq j\})$

    One then has, writing $\Delta X_{t_i} := X_{t_{i+1}} - X_{t_{i}} = \sum_{j \in [\xi(i),\xi(i+1)-1]} \Delta X_{s_j}$,
    \begin{align*}
        \norm{J_{\cD'} - J_{\cD}}_{\cH_K} &\leq
        \sum_{i \in [D]} 
        \norm{\sum_{j \in [\xi(i),\xi(i+1)-1]} K(X|_{[0,s_j]},\cdot)[\Delta X_{s_j}] - 
         K(X|_{[0,t_i]},\cdot)[\Delta X_{t_i}]}_{\cH_K}
        \\
        &\leq 
        \sum_{j\in [D']} 
        \norm{(K(X|_{[0,s_j]},\cdot) - K(X|_{[0,t_i]},\cdot))[\Delta X_{s_j}]}_{\cH_K}
        \\
        &\leq
        \sum_{j\in [D']} 
        \norm{K(X|_{[0,s_j]},\cdot) - K(X|_{[0,t_i]},\cdot)}_{\mathcal{L}(\bR^d, \cH_K)}
        \norm{\Delta X_{s_j}}_{\bR^d}
    \end{align*}

    \vspace{5pt}
    Consider now the map $G: [0,T] \to \mathcal{L}(\bR^d,\cH_K)$ defined as $G(s) = K(X|_{[0,s]},\cdot)$. This map is by hypotheses continuous on the compact $[0,T]$, thus it has a modulus of continuity $\omega_G$. Then
    
    \begin{align*}
        \norm{J_{\cD'} - J_{\cD}}_{\cH_{K}} &\leq
        \sum_{j\in [D']} 
        \norm{K(X|_{[0,s_j]},\cdot) - K(X|_{[0,t_i]},\cdot)}_{\mathcal{L}(\bR^d,\cH_{K})}
        \norm{\Delta X_{s_j}}_{\bR^d}
        \\
        &\leq
        \sum_{j\in [D']} 
        \omega_G(|s_{j} - s_{\tilde{\xi}(j)}|)
        \norm{\Delta X_{s_j}}_{\bR^d}
        \\
        &\leq
        \sum_{j\in [D']} 
        \omega_G(|\cD|)
        \norm{\Delta X_{s_j}}_{\bR^d}
        \leq
        \omega_G(|\cD|)
        \norm{X}_{1-var}
    \end{align*}

    From this, with classical arguments, follows that for any sequence of partitions $\cD_M$ of $[0,1]$ such that $|\cD_M| \to 0$ the sequence $J_{\cD_M}$ has a unique limit, which is independent of the chosen sequence. This defines the integral.
    Then (\ref{eqn:core_swap_1}) follows by a simple limit argument.
    % \footnote{\nico{We have to define the integral on the LHS first!}}
\end{proof}




\begin{proof}[more elegant Proof]
    Note how for any $(x,z) \in \Omega^\alpha\times \bR^d$
    \[
        \norm{K(x,\cdot)z}_{\cH_{K}}^2 = z^{\top} K(x,x)z = Tr(K(x,x)zz^{\top}) \leq |Tr(K(x,x))| Tr(zz^{\top}) = \norm{z}_{\bR^d}^2|Tr(K(x,x))|
    \]
    hence 
    \[
    \norm{K(x,\cdot)}_{\mathcal{L}(\bR^d;\cH_{K})}^2 \leq |Tr(K(x,x))|
    \]

    It follows that $\Phi_X$ is well defined in $L^2(*;\cH_{K})$ as a stochastic integral by \cite{??}.
    
    For any $f \in \cH_{K}$ the map $s \mapsto f(X|_{0,s})$ is clearly progressively measurable and the integral
    \[
    \int_0^T \left\langle f(X|_{[0,t]}), \D X_t \right\rangle_{\bR^d}
    \]
    is well defined since
    \[
    \norm{f(X|_{0,t})}^2_{\bR^d} \leq \norm{f}_{\cH_{K}}^2 Tr(K(X|_{0,t}, X|_{0,t}))
    \]
    hence
    \[
    \E\left[ \int_0^T \norm{f(X|_{0,t})}^2_{\bR^d} Tr(d[X,X]_t) \right]
    \leq
    \norm{f}_{\cH_{K}}^2 E\left[ \int_0^T Tr(K(X|_{0,t}, X|_{0,t})) Tr(d[X,X]_t) \right]
    \]
    thus the integral 
    \[
    \int_0^T \left\langle f(X|_{[0,t]}), \D X_t \right\rangle_{\bR^d} \in L^2(*;\bR)
    \]
    is well defined.

    By the commutativity of linear functionals and stochastic integration 
    \begin{align*}
        \int_0^T \left\langle f(X|_{[0,t]}), \D X_t \right\rangle_{\bR^d}
        = &  \int_0^T \sprod{f}{K(X|_{0,t},\cdot)\D X_t}
        \\
        =&  \sprod{f}{\int_0^T K(X|_{0,t},\cdot)\D X_t} = \sprod{f}{\Phi_X}
    \end{align*}
    
\end{proof}


\begin{lemma}
    Assume $X \in C^{\frac{1}{p}-\text{H\"o}}([0,T];\bR^d)$ for some $p \in [2, 3)$ with rough-path lift $\mathbf{X} = (X,\mathbb{X}): \Delta_{0,T} \to \bR^d \oplus (\bR^d)^{\otimes 2}$. Assume moreover
    \begin{equation}
       \{s \mapsto K(X)_s := K(X|_{[0,s]}, \cdot) \} \in C^{\frac{1}{p}-\text{H\"o}}([0,T];\cL(\bR^d, \cH_{K}))
    \end{equation}
    and the existence of a path 
    \begin{equation}
       K'(X) \in C^{\frac{1}{p}-\text{H\"o}}([0,T]; \cL(\bR^d, \cL(\bR^d, \cH_{K})))
    \end{equation}
    such that 
    \[
        K(X)_t - K(X)_s = K'(X)_s X_{s,t}  + R^{K}_{s,t}
    \]
    where it holds the bound $\norm{R^{K}}_{\frac{2}{p}} := \sup\limits_{s<t} \frac{|R^{K}_{s,t}|_{\cL(\bR^d, \cH_{K})}}{|t-s|^{\frac{2}{p}}} < \infty$.
    Then it is well defined in a rough sense 
    \[
        \Phi_X := \int_0^T K(X|_{[0,t]}, \cdot) d \mathbf{X}_t := \lim\limits_{|\mathcal{P}| \to 0} \sum\limits_{[s,t]\in \mathcal{P}}
        (K(X)_s X_{s,t} + K'(X)_s\mathbb{X}_{s,t}) \in \cH_{K}
    \]
    such that for any $f \in \cH_{K}$ in rough sense
    \begin{equation}\label{eqn:core_swap_rough}
        \int_0^T \left\langle f(X|_{[0,t]}), d \mathbf{X}_t \right\rangle_{\bR^d} = \left\langle f, \Phi_X \right\rangle_{\cH_{K}}
    \end{equation}
\end{lemma}
    
\begin{proof}
    The well definition of $\Phi_X$ is a consequence of \cite[Prop 1]{gubinelli2004controlling} stated as in \cite[Thm 4.10]{friz2020course}.
    Regarding the last statement note how
    \begin{align*}
        \norm{f(X|_{[0,t]}) - f(X|_{[0,s]})}_{\bR^d}
        &= \sup\limits_{\norm{z} \leq 1} |\sprod{f(X|_{[0,t]}) - f(X|_{[0,s]})}{z}_{\bR^d}|
        \\
        = &  \sup\limits_{\norm{z} \leq 1} |\sprod{f}{(K(X)_t - K(X)_s)z}_{\cH_{K}}|
        \\
        \leq &  \norm{f}_{\cH_{K}}  \sup\limits_{\norm{z} \leq 1}  \norm{(K(X)_t - K(X)_s)z}_{\cH_{K}}
        \\
        = &  \norm{f}_{\cH_{K}}^2  \norm{K(X)_t - K(X)_s}_{\cL(\bR^d, \cH_{K})}
    \end{align*}
    hence from the hypotheses $f(X|_{[0,s]}) \in C^{\frac{1}{p}-\text{H\"o}}([0,T]; \bR^d)$.
    
    Moreover
    \begin{align*}
        \sprod{f(X|_{[0,t]}) - f(X|_{[0,s]})}{z}_{\bR^d} 
        = &  \sprod{f}{(K(X)_t - K(X)_s)z}_{\cH_{K}}
        \\
        = &  \sprod{f}{(K'(X)_s X_{s,t}  + R^{K}_{s,t})z}_{\cH_{K}}
    \end{align*}
    thus if one defines the matrices and vectors
    \[
    [f'(X)_s]_i^j := \sprod{f}{(K'(X)_s e_j)e_i}_{\cH_{K}}
    \quad
    [R^{f}_{s,t}]_i := \sprod{f}{R^{K}_{s,t}e_i}_{\cH_{K}}
    \]
    one has
    \[
    f(X|_{[0,t]}) - f(X|_{[0,s]}) = f'(X)_s [X_{s,t}] + R^{f}_{s,t}
    \]
    where $f'(X)_s \in C^{\frac{1}{p}-\text{H\"o}}([0,T]; \bR^{d \times d})$ and $\norm{R^{f}_{s,t}}_{\frac{2}{p}} < \infty$
    since
    \begin{align*}
        \norm{f'(X)_t - f'(X)_s}_{op} 
        =&  \sup_{\norm{z}, \norm{y} \leq 1} |\sprod{f}{((K'(X)_t - K'(X)_s) z)y}_{\cH_{K}}|
        \\
        \leq & \norm{f}_{\cH_{K}} \norm{K'(X)_t - K'(X)_s}_{\cL(\bR^d, \cL(\bR^d, \cH_{K}))}
    \end{align*}
    and similarly
    \[
    \norm{R^{f}_{s,t}}_{\bR^d} \leq \norm{f}_{\cH_{K}} \norm{R^{K}_{s,t}}_{\cH_{K}}
    \]

    From these bounds one gets that the rough integral is well defined and\footnote{$A \odot B := Tr(AB)$}
    \begin{align*}
        \int_0^T \left\langle f(X|_{[0,t]}), d \mathbf{X}_t \right\rangle_{\bR^d} 
        = &  
        \lim\limits_{|\mathcal{P}| \to 0} \sum\limits_{[s,t]\in \mathcal{P}}
        \sprod{f(X|_{[0,s]})}{X_{s,t}}_{\bR^d} + f'(X)_s \odot \mathbb{X}_{s,t}
        \\
        = &  
        \lim\limits_{|\mathcal{P}| \to 0} \sum\limits_{[s,t]\in \mathcal{P}}
        \sprod{f}{K(X)_s X_{s,t}}_{\cH_{K}} + \sprod{f}{K'(X) \mathbb{X}_{s,t}}_{\cH_{K}}
        \\
        = &  
        \lim\limits_{|\mathcal{P}| \to 0} 
        \sprod{f}{\sum\limits_{[s,t]\in \mathcal{P}} K(X)_s X_{s,t} + K'(X) \mathbb{X}_{s,t}}_{\cH_{K}}
        \\ = & 
        \sprod{f}{\Phi_X}_{\cH_{K}}
    \end{align*}
\end{proof}



\begin{proposition}
    Let $p \geq 1$ and $N = \lfloor{p}\rfloor$. Assume $X \in C^{\frac{1}{p}-\text{H\"o}}([0,T];\bR^d)$ be a \textbf{geometric} rough-path with lift 
    $\mathbf{X} = (1, X^1,\cdots,X^N): \Delta_{0,T} \to T^N(\bR^d)$.
    Assume moreover the existence of a path 
    \[
    \boldsymbol{K}(X) = (K^0(X)_s, \cdots, K^{N-1}(X)_s) : [0,T] \to \bigoplus\limits_{k=0}^{N-1} \mathcal{L}((\bR^d)^{\otimes k}; \mathcal{L}(\bR^d; \cH_{K})) 
    \]
    extending $K(X)_s := K(X|_{[0,s]}, \cdot)$ ( \emph{i.e.} $K^0(X)_s = K(X)_s$ )
    and such that, for every word $I$ with $|I|\leq N - 1$ one has
    \begin{equation}
        \norm{\boldsymbol{K}(X)_t[e_I] - \boldsymbol{K}(X)_s[\mathbf{X}_{s,t} \otimes e_I]}_{\mathcal{L}(\bR^d; \cH_{K})} \leq C |t-s|^{(N-|I|)\frac{1}{p}}
    \end{equation}
    Then it is well defined in a rough sense 
    \[
        \Phi_X := \int_0^T K(X|_{[0,t]}, \cdot) d \mathbf{X}_t := \lim\limits_{|\mathcal{P}| \to 0} \sum\limits_{[s,t]\in \mathcal{P}}
        \sum_{|I| \leq N-1}\sum_{k =1}^d  (\boldsymbol{K}(X)_s[e_{I}])[e_k] \mathbf{X}^{Ik}_{s,t} \in \cH_{K}
    \]
    such that for any $f \in \cH_{K}$ in rough sense
    \begin{equation}\label{eqn:core_swap_rough}
        \int_0^T \left\langle f(X|_{[0,t]}), d \mathbf{X}_t \right\rangle_{\bR^d} = \left\langle f, \Phi_X \right\rangle_{\cH_{K}}
    \end{equation}
\end{proposition}

\begin{proof}
    The well definition of $\Phi_X$ is a consequence of \cite[Sect. 4.5]{friz2020course}.
    Regarding the last statement note how for any $z \in \bR^d$
    \begin{align*}
        \sprod{f(X|_{[0,t]})}{z}_{\bR^d} 
        = &  \sprod{f}{K(X)_t[z]}_{\cH_{K}}
        \\
        = & \sprod{f}{(\boldsymbol{K}(X)_t[e_{()}])[z]}_{\cH_{K}}
        \\
        = & \sprod{f}{(\boldsymbol{K}(X)_s[\mathbf{X}_{s,t}] + R^{f}_{s,t})[z]}_{\cH_{K}}
    \end{align*}
    where for all times $s,t$
    \[
    \norm{R^{f}_{s,t}}_{\mathcal{L}(\bR^d; \cH_{K})} \leq C|t-s|^{N\frac{1}{p}}
    \]

    Define then
    \begin{equation}
        \mathbf{f}(X) = (f^0(X), \cdots, f^{N-1}(X)): [0,T] \to  \bigoplus\limits_{k=0}^{N-1} \mathcal{L}((\bR^d)^{\otimes k}; \bR^d) 
    \end{equation}
    on the basis elements \[
    [f^{|I|}(X)_t[e_I]]_j := \sprod{f}{({K}^{|I|}(X)_t[e_I])[e_j]}_{\cH_{K}}
    \]

    and note how for every word $I$ with $|I|\leq N - 1$ one has
    \begin{align*}
        \norm{\boldsymbol{f}(X)_t[e_I] - \boldsymbol{f}(X)_s[\mathbf{X}_{s,t} \otimes e_I]}_{\bR^d} 
        = & \sup_{\norm{z} \leq 1} \sprod{\boldsymbol{f}(X)_t[e_I] - \boldsymbol{f}(X)_s[\mathbf{X}_{s,t} \otimes e_I]}{z}
        \\
        = & \sup_{\norm{z} \leq 1} \sprod{f}{\left(\boldsymbol{K}(X)_t[e_I] - \boldsymbol{K}(X)_s[\mathbf{X}_{s,t} \otimes e_I]\right)[z]}
        \\
        \leq & \norm{f}_{\cH_{K}} \norm{\boldsymbol{K}(X)_t[e_I] - \boldsymbol{K}(X)_s[\mathbf{X}_{s,t} \otimes e_I]}_{\mathcal{L}(\bR^d;\cH_{K})}
        \\
        \leq & \hspace{3pt} \norm{f}_{\cH_{K}} C |t-s|^{(N-|I|)\frac{1}{p}}
    \end{align*}
    
    
    From these bounds one gets that the rough integral is well defined and
    \begin{align*}
        \int_0^T \left\langle f(X|_{[0,t]}), d \mathbf{X}_t \right\rangle_{\bR^d} 
        := &  
        \lim\limits_{|\mathcal{P}| \to 0} \sum\limits_{[s,t]\in \mathcal{P}} \sum_{k =1}^d   \sum_{|I| \leq N-1} 
        \left[ \boldsymbol{f}(X)_s[e_{I}] \right]_k \mathbf{X}^{Ik}_{s,t}
        \\
        = &  
        \lim\limits_{|\mathcal{P}| \to 0} \sum\limits_{[s,t]\in \mathcal{P}} \sum_{|I| \leq N-1} \sum_{k =1}^d 
        \sprod{f}{(\boldsymbol{K}(X)_s[e_{I}])[e_k] \mathbf{X}^{Ik}_{s,t}}_{\cH_{K}}
        \\
        = &  
        \lim\limits_{|\mathcal{P}| \to 0} 
        \sprod{f}{\sum\limits_{[s,t]\in \mathcal{P}} \sum_{|I| \leq N-1} \sum_{k =1}^d 
        (\boldsymbol{K}(X)_s[e_{I}])[e_k] \mathbf{X}^{Ik}_{s,t}}_{\cH_{K}}
        \\ = & 
        \sprod{f}{\Phi_X}_{\cH_{K}}
    \end{align*}
\end{proof}


\begin{theorem}\label{thm:generic_Phi}
    Let $p \geq 1$ and $N = \lfloor{p}\rfloor$ and $x \in \cX$.
    If $\xi(x) \in C^{\frac{1}{p}-\text{H\"o}}([0,T]; \cH_{\xi})$ is a rough-path, \textbf{geometric} if $p \geq 3$, with lift 
    $$\boldsymbol{\xi}(x) = (1, {\xi}^1(x),\cdots,\xi^N(x)): \Delta_{0,T} \to T^N(\cH_{\xi})$$
    and there exists a path 
    \[
    \boldsymbol{K}(x) = (K^0(x), \cdots, K^{N-1}(x)) : [0,T] \to \bigoplus\limits_{m=0}^{N-1} \mathcal{L}(\cH_{\xi}^{\otimes m}; \mathcal{L}(\cH_{\xi}; \cH_{K})) 
    \]
    extending $K(x)_s := K(\psi(x)|_{[0,s]}, \cdot)$ ( \emph{i.e.} $K^0(x)_s = K(x)_s$ ) and such that, for every $m \leq N - 1$ one has
    \begin{equation}
        \norm{K^m(x)_t - \boldsymbol{K}(x)_s[\boldsymbol{\xi}(x)_{s,t} \otimes (\cdot)]}_{\mathcal{L}(\cH_{\xi}^{\otimes m}; \mathcal{L}(\cH_{\xi}; \cH_{K})) } \leq C |t-s|^{(N-m)\frac{1}{p}}
    \end{equation}
    \begin{equation}
        \norm{K^m(x)_t - K^m(x)_s}_{\mathcal{L}(\cH_{\xi}^{\otimes m}; \mathcal{L}(\cH_{\xi}; \cH_{K})) } \leq C |t-s|^{\frac{1}{p}}
    \end{equation}
    then it is well defined in a rough sense\footnote{we implicity use the inclusions $\mathcal{L}(\cH_{\xi}^{\otimes m}; \mathcal{L}(\cH_{\xi}; \cH_{K}))  \xhookrightarrow{} \mathcal{L}(\cH_{\xi}^{\otimes m +1}; \cH_{K})$.} 
    \begin{align*}
        \Phi_x & := \int_0^T K(\psi(x)|_{[0,t]}, \cdot) d \boldsymbol{\xi}(x)_t 
        \\
        & := \lim\limits_{|\mathcal{P}| \to 0} \sum\limits_{[s,t]\in \mathcal{P}}
        \sum_{m = 0}^{N-1}  K^m(x)_s [\boldsymbol{\xi}(x)^{m+1}_{s,t}]
        \in \cH_{K}
    \end{align*}
    such that for any $f \in \cH_{K}$ in the same rough sense
    \begin{equation}\label{eqn:core_swap_rough}
        \int_0^T \left\langle f(\psi(x)|_{[0,t]}), d \boldsymbol{\xi}(x)_t \right\rangle_{\cH_{\xi}} = \left\langle f, \Phi_x \right\rangle_{\cH_{K}}
    \end{equation}
\end{theorem}
\begin{proof}
    The well definition of $\Phi_X$ is a consequence of \cite[Thm. 4.10]{friz2020course} for $p < 3$, \cite[Sect. 4.5]{friz2020course} for $p\geq 3$.
    We use the notation of \cite[A.1]{roughFubini}. 
    Regarding the last statement, note how for any $z \in \cH_{K}$
    \begin{align*}
        \sprod{f(\psi(x)|_{[0,t]})}{z}_{\cH_{\xi}} 
        = &  \hspace{5pt}
        \sprod{f}{K(\psi(x)|_{[0,t]}, \cdot)z}_{\cH_{K}}
        \\
        = & \hspace{5pt}
        \sprod{f}{K^0(x)_t[1][z]}_{\cH_{K}}
        \\
        = & \hspace{5pt}
        \sprod{f}{\boldsymbol{K}(x)_s[\boldsymbol{\xi}(x)_{s,t}][z] + R^{f}_{s,t}[z]}_{\cH_{K}}
    \end{align*}
    where for all times $s,t$
    \[
    \norm{R^{f}_{s,t}}_{\mathcal{L}(\cH_{\xi}; \cH_{K})} \leq C|t-s|^{N\frac{1}{p}}
    \]

    This suggests to define
    \begin{equation}
        \mathbf{f}(x) = (f^0(x), \cdots, f^{N-1}(x)): [0,T] \to  \bigoplus\limits_{m=0}^{N-1} \mathcal{L}(\cH_{\xi}^{\otimes m}; \cH^*_{\xi}) 
    \end{equation}
    as
    \[
    \sprod{f^m(x)_t[v]}{z}_{\cH_{\xi}} := \sprod{f}{(K^m(x)_t[v])[z]}_{\cH_{K}}
    \]
    where $(v,z) \in \cH_{\xi}^{\otimes m} \times \cH_{\xi}$.
    Note then how for $m \leq N - 1$ and $v \in \cH_{\xi}^{\otimes m}$ one has
    \begin{align*}
        \norm{f^m(x)_t[v] - \boldsymbol{f}(x)_s[\boldsymbol{\xi}(x)_{s,t} \otimes v]}_{\cH_{\xi}^*} 
        = & \sup_{\norm{z} \leq 1} \sprod{f^m(x)_t[v] - \boldsymbol{f}(x)_s[\boldsymbol{\xi}(x)_{s,t} \otimes v]]}{z}_{\cH_{\xi}}
        \\
        = & \sup_{\norm{z} \leq 1} \sprod{f}{{K}^m(x)_t[v][z] - \boldsymbol{K}(x)_s[\boldsymbol{\xi}(x)_{s,t} \otimes v] [z]}_{\cH_{K}}
        \\
        \leq & \norm{f}_{\cH_{K}} \norm{{K}^m(x)_t[v] - \boldsymbol{K}(x)_s[\boldsymbol{\xi}(x)_{s,t} \otimes v ]}_{\mathcal{L}(\cH_{\xi};\cH_{K})}
    \end{align*}
    hence
    \begin{align*}
        \norm{f^m(x)_t - \boldsymbol{f}(x)_s[\boldsymbol{\xi}(x)_{s,t} \otimes (\cdot)]}_{\mathcal{L}(\cH_{\xi}^{\otimes m}; \cH_{\xi}^*)} 
        \leq & 
        \norm{f}_{\cH_{K}} \norm{{K}^m(x)_t - \boldsymbol{K}(x)_s[\boldsymbol{\xi}(x)_{s,t} \otimes (\cdot)]}_{\mathcal{L}(\cH_{\xi}^{\otimes m}; \mathcal{L}(\cH_{\xi};\cH_{K}))}
        \\
        \leq & \hspace{3pt} \norm{f}_{\cH_{K}} C |t-s|^{(N-m)\frac{1}{p}}
    \end{align*}

    Similarly
    \begin{align*}
        \norm{f^m(x)_t[v] - f^m(x)_s[v]}_{\cH_{\xi}^*}
        = & 
        \sup_{\norm{z} \leq 1} 
        \sprod{f^m(x)_t[v] - f^m(x)_s[v]}{z}_{\cH_{\xi}}
        \\
        = & 
        \sup_{\norm{z} \leq 1} 
        \sprod{f}{(K^m(x)_t - K^m(x)_s)[v][z]}_{\cH_{K}}
        \\
        \leq & 
        \norm{f}_{\cH_{K}} \norm{K^m(x)_t - K^m(x)_s} \norm{v}_{\cH_{\xi}^{\otimes m}}
        \\
        \leq & 
        \norm{f}_{\cH_{K}} C |t-s|^{\frac{1}{p}} \norm{v}_{\cH_{\xi}^{\otimes m}}
    \end{align*}
    thus similarly to before we get the bound
    \[
    \norm{f^m(x)_t - f^m(x)_s}_{\mathcal{L}(\cH_{\xi}^{\otimes m}; \cH_{\xi}^*)} \leq \norm{f}_{\cH_{K}} C |t-s|^{\frac{1}{p}} 
    \]
    
    From these bounds one gets that the rough integral is well defined and, using the inclusions $\mathcal{L}(\cH_{\xi}^{\otimes m}; \mathcal{L}(V; W))\xhookrightarrow{} \mathcal{L}(\cH_{\xi}^{\otimes m} \otimes V; W)$ and $\mathcal{L}(\cH_{\xi};\bR) = \cH_{\xi}^*$, we have
    \begin{align*}
        \int_0^T \left\langle f(\psi(x)|_{[0,t]}), d \boldsymbol{\xi}(x)_t \right\rangle_{\cH_{\xi}} 
        := &  
        \lim\limits_{|\mathcal{P}| \to 0} \sum\limits_{[s,t]\in \mathcal{P}} 
        \sum_{m=0}^{N-1} f^m(x)_s[\boldsymbol{\xi}(x)_{s,t}^{m+1}]
        \\
        = &  
        \lim\limits_{|\mathcal{P}| \to 0} \sum\limits_{[s,t]\in \mathcal{P}} \sum_{m=0}^{N-1}
        \sprod{f}{K^m(x)_s[\boldsymbol{\xi}(x)_{s,t}^{m+1}]}_{\cH_{K}}
        \\
        = &  
        \lim\limits_{|\mathcal{P}| \to 0} 
        \sprod{f}{
        \sum\limits_{[s,t]\in \mathcal{P}} \sum_{m=0}^{N-1}
        K^m(x)_s[\boldsymbol{\xi}(x)_{s,t}^{m+1}]}_{\cH_{K}}
        \\ = & \hspace{5pt}
        \sprod{f}{\Phi_x}_{\cH_{K}}
    \end{align*}
\end{proof}
